A Baseline for Shapley Values in MLPs: from Missingness to Neutrality

Deep neural networks have gained momentum based on their accuracy, but their interpretability is often criticised. As a result, they are labelled as black boxes. In response, several methods have been proposed in the literature to explain their predictions. Among the explanatory methods, Shapley values is a feature attribution method favoured for its robust theoretical foundation. However, the analysis of feature attributions using Shapley values requires choosing a baseline that represents the concept of missingness. An arbitrary choice of baseline could negatively impact the explanatory power of the method and possibly lead to incorrect interpretations. In this paper, we present a method for choosing a baseline according to a neutrality value: as a parameter selected by decision-makers, the point at which their choices are determined by the model predictions being either above or below it. Hence, the proposed baseline is set based on a parameter that depends on the actual use of the model. This procedure stands in contrast to how other baselines are set, i.e. without accounting for how the model is used. We empirically validate our choice of baseline in the context of binary classification tasks, using two datasets: a synthetic dataset and a dataset derived from the financial domain.

==> 2-Background.tex <==
In this section we review the relevant background material and the literature related to our work.

\subsection{Shapley Values and Their Baselines}

%Shapley values for explainability in ML have been introduced by \cite{lundberg2017unified}. 
For a neural network $G_{\theta}$ with parameters $\theta$, and $K$ input features, the contribution of feature $j$ calculated according to the Shapley value for input $x=[x_1, x_2, \dots, x_K]$ %\todo{Do we consider a bias term in the features?} 
is given by:
\begin{equation}%\nonumber
\sum_{S \subseteq P \setminus \{j\}} \frac{|S|!(|P|-|S|-1)!}{|P|!}\left(
G_{\theta}(\tilde{x}_{S \cup \{j\}}) - 
G_{\theta}(\tilde{x}_{S})\right),
\end{equation}
%$x_S$ is observation $x$ with all elements in $S$ set to the observation value, and the rest set to  the respective baselines: $b_{P \setminus S}$.
%
%Where the sum goes over all possible combinations of features without feature $j$. 
%
%where an element of $\tile{x}_S$, let say $\tilde{x}_{S,i}$, is given by $\tilde{x}_{S,i}=x_i1_{i\in S}$
where $P$ is the collection of all feature indexes, element $i$ of vector $\tilde{x}_S$ is given by $\tilde{x}_{S,i}=x_i \mathbbm{1}_{\{i\in S\}} + b_i \mathbbm{1}_{\{i \not\in S\}}$ (similarly for $\tilde{x}_{S\cup \{j\}}$), and $b_i$ is the baseline value for feature $i$. The \textit{baseline} models the missingness of a feature, i.e., it replaces that feature when it is absent. As it is argued by \cite{sturmfels2020visualizing}, unlike game theory, the concept of missingness is not well defined and explored in ML models. Some authors \textcolor{red}{(Citations needed)} address the issue by removing the feature(s) from the model via marginalization, thus assuming a distribution for $b_i$. Nevertheless, the standard practice in setting up a baseline is to assign a vector of zeros for all features. However, this choice might provide wrong interpretations and even give zero importance to significant features. % \citealp{sturmfels2020visualizing}.

On the other hand, as the number of features increases, calculating Shapley values becomes expensive as the computational cost is exponential with respect to the number of features. Hence, estimation methods have been developed, and the most commonly used ones in Deep Learning are 
Deep Taylor Decomposition \cite{Montavon2017a}, 
Integrated Gradient \cite{Sundararajan2017}, 
Deep SHAP \cite{lundberg2017unified}, and
Deep LIFT \cite{shrikumar2017learning}. 
Other model agnostic methods are:
Sampled and Kernel SHAP \cite{castro2009polynomial,strumbelj2010efficient, datta2016algorithmic,lundberg2017unified,okhrati2020multilinear}.

All of these methods require a choice to be made on the baseline to use. In the next section, we review commonly used methods in choosing a baseline.

\subsection{The Choice of a Baseline}

As mentioned earlier, the simplest choice of a baseline is the \textbf{zero} vector baseline \cite{zeil2014,Sundararajan2017,shrikumar2017learning,Ancona2019}, which coincides with the \textbf{average} vector baseline when features are standardized. However, this choice could be misleading. 

One way of addressing the zero-baseline insensitivity problem %mentioned earlier 
is to use the maximum distance baseline (\textbf{mdb}) method as in \cite{sturmfels2020visualizing}. 
This baseline consists in taking the furthest observation from the current one in an $L^1$ norm. However, this approach unequivocally creates incoherent justifications for the interpretations provided by the model due to the high correlation of the baseline with the underlying dataset.

Alternatively, one can sample a baseline from a multivariate distribution such as uniform \cite{sturmfels2020visualizing} or Gaussian \cite{smilkov2017smoothgrad}. This approach can be improved by considering a sample of baselines and to average the attributions computed over each baseline % \textcolor{red}{randomly drawn baselines}, 
\cite{smilkov2017smoothgrad,lundberg2017unified,erion2019learning,kapishnikov2019xrai,sundararajan2019many}. 
Another form of sampling is the one performed using the dataset. 
Hence, one can use the underlying empirical distributions of the dataset \cite{lundberg2017unified,sundararajan2019many,sturmfels2020visualizing}. We denote this as the \textbf{p}$_{X}$ baseline method. However, the \textbf{p}$_{X}$ baseline increases the computational cost of estimating feature attributions linearly with respect to the number of draws. Further, the expectation over a run on multiple baselines could be a reasonable option to compute feature importance, but ranking features in order of importance is not the only purpose of an explainability method.
%Most of the time the end-user of the model wants, in addition to the latter, to be able to interpret the feature attribution with respect to threshold 

For the Deep Taylor Decomposition approach, the baselines are chosen using Layer-wise Relevance Propagation \cite{Bach2015} or Pattern Attribution \cite{kindermans2017learning}. The drawback of these baseline search methods is the non applicability %their limitation  of being applicable only to DTD, and not applicable 
to other attribution methods, such as exact Shapley values or Shapley sampling. For this reason we do not compare against them. 


% or Integrated Gradient methods.
%Nevertheless, in \cite{Bach2015} many methods are proposed to find neutral baselines for a Taylor-type decomposition. All of those look for a baseline that delivers to a neutral output and it is close to the current observation with respect to some distance. As with the maximum distance approach, this would provide baselines which are highly correlated with the data. In the empirical section, we will implement this method and use the Euclidean norm as a measure of the distance with respect to the current observation (\textbf{neutral$_{||^2}$}). Further, as suggest by the authors, when there are multiple solutions per observation, we will average the contributions computed over the solutions found.
%In the following section, we discuss our methodology and in particular compare it with \textbf{zero}, \textbf{average}, 
%\textbf{p}$_{X}$, and 
%\textbf{mdb} baselines. \todo{We need to explain briefly either here or in the introduction that how our method differentiates from the above ones and to explain its pros and cons.}

% In \cite{sturmfels2020visualizing} several methods are discussed: the Uniform baseline (random baseline from a Uniform distribution), the Gaussian baseline (add random noise from a Normal distribution), 

%  For the random baselines, the authors suggest 


\subsection{Measure of Explainability Power}

The evaluation of explainability methods from a quantitative perspective is difficult due to the lack of a clear definition of what is a correct explanation \cite{samek2016evaluating,Sundararajan2017,Ancona2019}.
%
Many extrinsic evaluation of explainability power have been developed. These are based on measuring the effect on a model when removing the most important feature as identified by a feature attribution method. Some quantify this effect by measuring the difference in performance \cite{hooker2019benchmark}, and others by measuring the difference in prediction value \cite{Anconaetal2017}. % feature based on  between the performance (or prediction) of a model using a set of features  sets of features. In particular, these measure when different sets of features are used and when a set of these are masked based on how important the feature attribution method has judged them. 
The intuition behind these methods is that if the feature attribution method correctly identifies the most important feature, then when this feature is removed, the model performance should decrease more (or the prediction value should deviate more) than when a less important feature is removed. In this paper, we use these evaluation methods %originally developed for feature attribution methods 
to compare %instead, using the same attribution method, 
the choice of baselines.
%
A limitation of these evaluation methods is that since a feature is removed once at the time, these measures may be mislead by potential feature correlations. In this paper, to avoid this issue, we also perform an analysis using a synthetic dataset where features are generated independently.

%While the ultimate purpose of an explainability method is domain specific, we argue that there are at least two desiderata that the method should satisfy. First of all, it must rank the feature importance correctly. Second, it must be directly interpretable to the end user. 

%These evaluation methods can be applied \textit{globally} or \textit{locally}. 
%They are global when the discovery of the most important feature is done by analysing a large sample of data points. While, these methods are local when the discovery of the most important feature is done on a per example basis. \citet{hooker2019benchmark} propose a global measure called RemOve And Retrain (ROAR). %as introduced by 
%%In this paper we use the method introduced 
%This consists in, given a model, to first identify the most important feature using the whole dataset, then retrain the model without this feature and measure the difference in performance between the two models. 
%\citet{Anconaetal2017} proposed a measure of local evaluation %we find inspiration on the 
%proposed ROAR to measure the goodness of interpretability methods. ROAR consists ...
%
%However, this method has the drawback ... of this method for dependent features, 
%
%method proposed by
%which consists in, given a model, %for each data point, 
%to first identify the most important feature for each example, then removing this feature by substituting it with its baseline value and measure the deviation in prediction. These deviations are then averaged to get a single value. %MEan Rebase and Evaluate


%proposed a perturbation test where most important features are removed and replaced with the baseline. 
%In principle, for a given classification problem, a model with all the features removed should be considered as uninformative. 

